Learning Linear Models Using Distributed Iterative Hessian Sketching

This work considers the problem of learning the Markov parameters of a linear system from observed data. Recent non-asymptotic system identification results have characterized the sample complexity of this problem in the single and multi-rollout setting. In both instances, the number of samples required in order to obtain acceptable estimates can produce optimization problems with an intractably large number of decision variables for a second-order algorithm. We show that a randomized and distributed Newton algorithm based on Hessian-sketching can produce $\epsilon$-optimal solutions and converges geometrically. Moreover, the algorithm is trivially parallelizable. Our results hold for a variety of sketching matrices and we illustrate the theory with numerical examples.

==> introduction.tex <==
% introduction
Neural networks have been successfully applied in system identification to model complex nonlinear dynamics with high accuracy. Despite its outstanding predictive power, the complex structure of neural networks brings significant challenge in analyzing the reachability of the neural network system. For a feedforward fully connected neural network, the reachability analysis is NP-hard, hence convex relaxation-based methods have been proposed to compute over-approximations of the reachable sets of a neural network system which try to strike a balance between conservatism in the over-approximation and computational efficiency.

First, we introduce the LP-based relaxation for the output set approximation of a feedforward fully connected neural network. For finite-step reachability analysis, we demonstrate that applying the LP-based relaxation on the $k$-step composition of the NN gives tighter over-approximation than applying the same relaxation $k$ times. We refer to the first method as \emph{sequential LP-relaxation} and the second one as \emph{iterative LP-relaxation}. We prove that the sequential method is always less conservative than the iterative one which is confirmed through numerical examples.

Second, we compare sequential vs. iterative approaches with other weaker but faster LP-based relaxation methods and show that the edge of the sequential method over the iterative method is not guaranteed with these weaker relaxations.

Finally, we present how to apply ADMM to solve the exact LP-based relaxation and demonstrate that with GPU acceleration, ADMM can achieve 7x speedup compared with commercial LP solvers such as Gurobi. This highlights the scalability of our proposed method and its potential in long-scope or large-scale neural network system reachability analysis. 


